Principal-Agent Boolean Games

We introduce and study a computational version of the principal-agent problem -- a classic problem in Economics that arises when a principal desires to contract an agent to carry out some task, but has incomplete information about the agent or their subsequent actions. The key challenge in this setting is for the principal to design a contract for the agent such that the agent's preferences are then aligned with those of the principal. We study this problem using a variation of Boolean games, where multiple players each choose valuations for Boolean variables under their control, seeking the satisfaction of a personal goal, given as a Boolean logic formula. In our setting, the principal can only observe some subset of these variables, and the principal chooses a contract which rewards players on the basis of the assignments they make for the variables that are observable to the principal. The principal's challenge is to design a contract so that, firstly, the principal's goal is achieved in some or all Nash equilibrium choices, and secondly, that the principal is able to verify that their goal is satisfied. In this paper, we formally define this problem and completely characterise the computational complexity of the most relevant decision problems associated with it.

==> Figures/2_player_game.tex <==
\begin{tikzpicture}
    \begin{scope}
%% Draw rectangles
    \draw[fill=blue, fill opacity = 0.05, rounded corners] (-3,3) rectangle (7,-3);
    % \draw[fill=blue, fill opacity = 0.1, draw = black, rounded corners] (-4, 4) rectangle (5, -1.5);
    % \draw[fill=blue, fill opacity = 0.15, draw = black, rounded corners] (-3, 3) rectangle (4, -1);
    % \draw[fill=blue, fill opacity = 0.15, rounded corners] (-2, 2) rectangle (3, -0.5);
    % \draw[fill=blue, fill opacity = 0.15, rounded corners] (-1, 1) rectangle (2, 0);
%% Add text
    \end{scope}
    
    \filldraw[blue] (0,0) circle (2pt) node[anchor=west]{Intersection point};
    \filldraw[blue] (1,1) circle (2pt) node[anchor=west]{Intersection point};
    \filldraw[blue] (1,1) circle (2pt) node[anchor=west]{Intersection point};
    \filldraw[blue] (1,1) circle (2pt) node[anchor=west]{Intersection point};
    
    \node[text=black] at (-4.5,4.5) {\huge$\Omega$};
    \node[text=black] at (0.5,3.5) {\huge$MCDT(G)$};
    \node[text=black] at (0.5,2.5) {\huge$wMCD(G)$};
    \node[text=black] at (0.5,1.5) {\huge$MCD(G)$};
    \node[text=black] at (0.5,0.5) {\huge$SCD(G)$};
\end{tikzpicture}

